Privacy-preserving Logistic Regression with Secret Sharing

Logistic regression (LR) is a widely used classification method for modeling binary outcomes in many medical data classification tasks. Research that collects and combines datasets from various data custodians and jurisdictions can excessively benefit from the increased statistical power to support their analyzing goals. However, combining data from these various sources creates significant privacy concerns that need to be addressed. In this paper, we proposed secret sharing-based privacy-preserving logistic regression protocols using the Newton-Raphson method. Our proposed approaches are based on secure Multi-Party Computation (MPC) with different security settings to analyze data owned by several data holders. We conducted experiments on both synthetic data and real-world datasets and compared the efficiency and accuracy of them with those of an ordinary logistic regression model. Experimental results demonstrate that the proposed protocols are highly efficient and accurate. This study introduces iterative algorithms to simplify the federated training a logistic regression model in a privacy-preserving manner. Our implementation results show that our improved method can handle large datasets used in securely training a logistic regression from multiple sources.

==> TableFigure.tex <==
\textbf{\large Additional files} 

\bigskip
All data are free and publicly available:
\medskip

\begin{itemize}
    \item \textbf{pcs.csv}, Prostate CancerStudy (PCS), A subset of data from a study of patient with prostate cancer. Variables measured at the baseline patient exam were used to try to determine whether the tumor had penetrated the prostate capsule. 
    \item \textbf{lbw.csv}, Low Birth Weight study data (LBW), This data was collected as part of a larger study at Bayside Medical Center, Springfield, Massachusetts. It contains information on 189 births to women that were seen in the obsetetrics clinic. 
 
    \item \textbf{uis.csv}, UMARU IMPACT Study data (UIS), A subset of data from the University of Massachusetts Aids Research Unit (UMARU) IMPACT study. This came from two parallel randomized trials of residential treatment for drug abuse to compare the planned duration of admission. 
    
    \item \textbf{pima.csv}, Pima Indians Diabetes (PIMA), This dataset is originally from the National Institute of Diabetes and Digestive and Kidney Diseases. The objective of the dataset is to diagnostically predict whether or not a patient has diabetes based on specific diagnostic measurements included in the dataset.
\end{itemize}





\clearpage

\textbf{\large Table and Figure Legends}


\begin{table}[H]
\centering
\caption{Memory consumption comparison of our proposed protocols using generated synthetic datasets}
\label{memory}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\begin{tabular}[c]{@{}c@{}}Records\\Number\end{tabular} & \begin{tabular}[c]{@{}c@{}}Feature\\Number\end{tabular} & \begin{tabular}[c]{@{}c@{}}OLR\\\end{tabular} & BMPC & CMPC & \begin{tabular}[c]{@{}c@{}}Accurate\\BMPC~\end{tabular} & \begin{tabular}[c]{@{}c@{}}Accurate\\CMPC\end{tabular} \\ 
\hline
10000 & 50 & 3666 & 1325 & 688 & 1316 & 888 \\ 
\hline
20000 & 70 & 12559 & 1717 & 1016 & 1665 & 1325 \\ 
\hline
30000 & 90 & 22736 & 2743 & 1702 & 2654 & 2033 \\ 
\hline
40000 & 100 & 29110 & 3775 & 2337 & 3622 & 2672 \\ 
\hline
50000 & 100 & 34394 & 4575 & 2878 & 4406 & 3220 \\ 
\hline
50000 & 200 & 34512 & 8516 & 5437 & 8013 & 5770 \\
\hline
\end{tabular}
\end{table}




\begin{table} [H]
\centering
\caption{A comparison between model parameters $\beta$ learned using the proposed protocols and ordinary logistic regression protocol over LBW dataset}
\label{tab_accurate_beta}
\begin{tabular}{cccccccclc} 
\toprule
\multirow{2}{*}{$\beta$} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Ordinary \\LR\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Accurate \\BMPC\end{tabular}} & \multicolumn{3}{c}{BMPC} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Accurate\\CMPC\\\end{tabular}} & \multicolumn{3}{c}{CMPC} \\ 
\cmidrule{4-6}\cline{8-10}
 &  &  & 3 & 5 & 7 &  & 3 & \multicolumn{1}{c}{5} & 7 \\ 
\hline
$\beta_1$ & 0.01574 & 0.01577 & 0.01761 & 0.01580 & 0.01480 & 0.01574 & 0.02214 & 0.01793 & 0.01630 \\
$\beta_2$ & 0.01127 & 0.01123 & 0.01171 & 0.01061 & 0.01006 & 0.01127 & 0.01534 & 0.01266 & 0.01166 \\
$\beta_3$ & 0.78666 & 0.78152 & 0.67763 & 0.62479 & 0.60392 & 0.78662 & 0.95081 & 0.81191 & 0.77010 \\
$\beta_4$ & -0.47132 & -0.46992 & -0.48975 & -0.44423 & -0.42170 & -0.47131 & -0.63960 & -0.52621 & -0.48340 \\
$\beta_5$ & -1.32410 & -1.31870 & -1.24442 & -1.13786 & -1.08974 & -1.32405 & -1.68676 & -1.41595 & -1.32408 \\
$\beta_6$ & -0.75584 & -0.75594 & -0.86971 & -0.78142 & -0.73330 & -0.75583 & -1.09894 & -0.88944 & -0.80596 \\
$\beta_7$ & -2.20748 & -2.20104 & -2.48191 & -2.23117 & -2.09511 & -2.20743 & -3.15262 & -2.56252 & -2.33208 \\
$\beta_8$ & -0.96060 & -0.95756 & -0.99906 & -0.90459 & -0.85667 & -0.96058 & -1.30317 & -1.07358 & -0.98838 \\
$\beta_9$ & -0.24569 & -0.24476 & -0.21884 & -0.20160 & -0.19465 & -0.24568 & -0.30509 & -0.25879 & -0.24367 \\
\bottomrule
\end{tabular}
\end{table}



\begin{table}[H]
\centering
\caption{Accuracy comparison result for real-word datasets with different settings}
\label{accuracy_table}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\cline{5-10}
\multicolumn{1}{c}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}CMPC \end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}BMPC \end{tabular}} & \multicolumn{2}{c|}{OLR} \\ 
\hline
Dataset & \begin{tabular}[c]{@{}c@{}}Records\\Num \end{tabular} & \begin{tabular}[c]{@{}c@{}}Feature\\Num \end{tabular} & \begin{tabular}[c]{@{}c@{}}g(x) \\degree \end{tabular} & Accuracy & AUC & \multicolumn{1}{l|}{Accuracy} & AUC & \multicolumn{1}{r|}{Accuracy} & \multicolumn{1}{l|}{AUC} \\ 
\hline
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & 3 & 71.87\% & \multicolumn{1}{r|}{0.740} & 71.87\% & 0.740 & 71.87\% & 0.740 \\ 
\cline{4-10}
\multirow{2}{*}{PIMA} & \multirow{2}{*}{768} & \multirow{2}{*}{9} & 5 & 71.87\% & \multicolumn{1}{r|}{0.741} & 71.87\% & 0.740 & 71.87\% & 0.740 \\ 
\cline{4-10}
 &  &  & 7 & 71.87\% & \multicolumn{1}{l|}{0.741} & 71.87\% & 0.741 & 71.87\% & 0.741 \\ 
\cline{4-10}
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & No approx & - & - & - & - & 71.87\% & 0.741 \\ 
\hline
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & 3 & 81.05\% & \multicolumn{1}{r|}{0.842} & 81.05\% & 0.846 & 80\% & 0.846 \\ 
\cline{4-10}
\multirow{2}{*}{PCS} & \multirow{2}{*}{379} & \multirow{2}{*}{10} & 5 & 81.05\% & \multicolumn{1}{r|}{0.845} & 81.05\% & 0.847 & 80\% & 0.847 \\ 
\cline{4-10}
 &  &  & 7 & 81.05\% & \multicolumn{1}{l|}{0.847} & 81.05\% & 0.848 & 81.05\% & 0.848 \\ 
\cline{4-10}
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & No approx & - & - & - & - & 81.05\% & 0.848 \\ 
\hline
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & 3 & 64.58\% & 0.519 & 64.58\% & 0.519 & 64.58\% & \multicolumn{1}{l|}{0.519} \\ 
\cline{4-10}
\multirow{2}{*}{LBW} & \multirow{2}{*}{189} & \multirow{2}{*}{10} & 5 & 64.58\% & \multicolumn{1}{r|}{0.519} & 64.58\% & 0.519 & 64.58\% & \multicolumn{1}{l|}{0.519} \\ 
\cline{4-10}
 &  &  & 7 & 62.5\% & \multicolumn{1}{l|}{0.519} & 62.5\% & 0.517 & 64.58\% & \multicolumn{1}{l|}{0.519} \\ 
\cline{4-10}
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & No approx & - & - & - & - & 62.5\% & 0.523 \\ 
\hline
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & 3 & 73.61\% & 0.651 & 73.61\% & 0.651 & 73.61\% & \multicolumn{1}{l|}{0.651} \\ 
\cline{4-10}
\multirow{2}{*}{UIS} & \multirow{2}{*}{575} & \multirow{2}{*}{9} & 5 & 72.91\% & \multicolumn{1}{r|}{0.652} & 72.91\% & 0.652 & 72.91\% & \multicolumn{1}{l|}{0.652} \\ 
\cline{4-10}
 &  &  & 7 & 72.91\% & 0.655 & 73.61\% & \multicolumn{1}{l|}{0.651} & 72.91\% & \multicolumn{1}{l|}{0.655} \\ 
\cline{4-10}
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & No approx & - & - & - & - & 72.22\% & 0.656 \\
\hline
\end{tabular}
\end{table}

\newpage

